Non-linear Higgs portal to Dark Matter

The Higgs portal to scalar Dark Matter is considered in the context of non-linearly realised electroweak symmetry breaking. We determine the dominant interactions of gauge bosons and the physical Higgs particle $h$ to a scalar singlet dark matter candidate. Phenomenological consequences are also studied in detail, including the possibility of distinguishing this scenario from the standard Higgs portal in which the electroweak symmetry breaking is linearly realised. Two features of significant impact are: i) the connection between the electroweak scale $v$ and the Higgs particle departs from the $(v+h)$ functional dependence, as the Higgs field is not necessarily an exact electroweak doublet; ii) the presence of specific couplings that arise at different order in the non-linear and in the linear expansions. These facts deeply affect the dark matter relic abundance, as well as the expected signals in direct and indirect searches and collider phenomenology, where Dark Matter production rates are enhanced with respect to the standard portal.

==> Fdiagrams/monoH_linear.tex <==

\begin{fmffile}{Fdiagrams/monoH_linear}
\parbox[c][3cm]{4.5cm}{\centering
\begin{fmfgraph*}(130,70)	% S in t-channel
\fmfleft{i1,i2}
\fmfright{o3,o2,o1}
\fmfset{arrow_len}{3mm}
  \fmf{gluon}{i2,v1}
  \fmf{gluon}{i1,v2}
  \fmf{fermion,tension=.7}{v1,v2,v3,v1}
  \fmf{dashes,lab=$h$,tension=.75,l.side=left}{v3,v4}
  \fmf{dashes}{v4,o1}
  \fmf{dashes}{v4,o2}
  \fmf{dashes}{v4,o3}   
   
\fmfv{lab=$h$,l.angle=0}{o1}
\fmfv{lab=$S$,l.angle=0}{o2}
\fmfv{lab=$S$,l.angle=0}{o3}
\fmfv{lab=$g$,l.angle=180}{i1}
\fmfv{lab=$g$,l.angle=180}{i2}

\fmfv{lab=$t$,l.angle=120,l.dist=10}{v3}
%\fmfv{lab={\scriptsize$\lambda_{Sh}$},l.angle=-125}{v4}

\end{fmfgraph*}
}
\end{fmffile}

